Hierarchies of Relaxations for Online Prediction Problems with Evolving Constraints

We study online prediction where regret of the algorithm is measured against a benchmark defined via evolving constraints. This framework captures online prediction on graphs, as well as other prediction problems with combinatorial structure. A key aspect here is that finding the optimal benchmark predictor (even in hindsight, given all the data) might be computationally hard due to the combinatorial nature of the constraints. Despite this, we provide polynomial-time \emph{prediction} algorithms that achieve low regret against combinatorial benchmark sets. We do so by building improper learning algorithms based on two ideas that work together. The first is to alleviate part of the computational burden through random playout, and the second is to employ Lasserre semidefinite hierarchies to approximate the resulting integer program. Interestingly, for our prediction algorithms, we only need to compute the values of the semidefinite programs and not the rounded solutions. However, the integrality gap for Lasserre hierarchy \emph{does} enter the generic regret bound in terms of Rademacher complexity of the benchmark set. This establishes a trade-off between the computation time and the regret bound of the algorithm.

==> notation.tex <==
\newcommand{\Dcal}{\mathcal{D}}

\newcommand{\A}{\mathbf{A}}

\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\z}{z}
\newcommand{\bz}{\mbf{z}}
%\def\mathbi#1{\textbf{\em #1}}
\def\mathbi#1{{\bm #1}}
\newcommand{\tz}{\mathbi{z}}
\newcommand{\tx}{\mathbi{x}}
\renewcommand{\th}{\mathbi{h}}
\newcommand{\ts}{\mathbi{s}}
\newcommand{\tv}{\mathbi{v}}
\newcommand{\tu}{\mathbi{u}}
\newcommand{\ty}{\mathbi{y}}
\newcommand{\ta}{\mathbi{a}}
\newcommand{\mbi}{\mathbi}
\newcommand{\ol}[1]{{\tilde{#1}}}
\newcommand{\rn}{{\Re^n}}
\newcommand{\popt}{p^\star}
\newcommand{\qopt}{q^\star}
\newcommand{\w}{\ensuremath{\mathbf{w}}}
\newcommand{\h}{\ensuremath{\mathbf{h}}}
%\newcommand{\h}{h}
\renewcommand{\v}{\ensuremath{\mathbf{v}}}
\newcommand{\xa}{\ensuremath{\mathbf{a}}}
%\newcommand{\W}{\ensuremath{\mathbf{W}}}
\newcommand{\Hy}{\ensuremath{\mathcal{H}}}
\newcommand{\x}{\ensuremath{\mathbf{x}}}
\newcommand{\loss}{\ell}
\newcommand{\empF}{\hat{F}}
\newcommand{\empL}{\hat{L}}
\newcommand{\wml}{\hat{\w}} % w minimizing training regularized objective
\newcommand{\moff}{m_{\mrm{off}}}
\newcommand{\mon}{m_{\mrm{online}}}
\newcommand{\mstat}{m_{\mrm{stat}}}

\newcommand{\eps}[1]{\epsilon_{\mathrm{#1}}}

\newcommand{\epscon}{\eps{cons}}
\newcommand{\epsempp}{\eps{emp}}
\newcommand{\epsapprox}{\eps{erm}}
\newcommand{\epsstable}{\eps{stable}}
\newcommand{\epsgen}{\eps{gen}}
\newcommand{\epspgen}{\eps{oag}}

\newcommand{\wopt}{\w^{\star}} % w minimizing regularized gen error

\newcommand{\hopt}{\h^{\star}}

\newcommand{\hemp}{\hat{\h}}
\newcommand{\J}{\mbf{J}}

\newcommand{\wref}{\w_{o}} % orcacle given predictor

\newcommand{\walgo}{\tilde{\w}} % w by algorithm

\newcommand{\wonline}{\w}

%\newcommand{\F}{\mathcal{F}}
\newcommand{\F}{{L}}

\newcommand{\tF}{\mathcal{\tilde{L}}}
\newcommand{\tL}{\mathcal{\tilde{L}}}
\newcommand{\tf}{\tilde{\ell}}
\newcommand{\tl}{\tilde{\ell}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Lip}{L}
\newcommand{\Lipf}{L}
\newcommand{\Lipff}{L_{\ff}}
\newcommand{\Liprr}{L_{\rr}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\LL}{{\cal L}}
\newcommand{\Bw}{B}
\newcommand{\Bphi}{R}
\newcommand{\ff}{g}
\newcommand{\rr}{r}
\newcommand{\e}{\mathbf{e}}

\newcommand{\U}{\mathcal{U}}  %  Bound on norm of X

\newcommand{\Ref}{R_{ref}}  %  Norm of Wref
\newcommand{\opterr}{\epsilon_{\mathrm{opt}}}



\newcommand{\y}{\mathbf{y}}
%\newcommand{x}{R}

\newcommand{\rate}{\epsilon}

\newcommand{\fcx}{\ell_{\eqref{eq:fcx}}}
\newcommand{\Fcx}{L_{\eqref{eq:fcx}}}
\newcommand{\empFcx}{\empL_{\eqref{eq:fcx}}}
\newcommand{\fcxx}{\ell_{\eqref{eq:fcxx}}}
\newcommand{\Fcxx}{\L_{\eqref{eq:fcxx}}}
\newcommand{\empFcxx}{\empL_{\eqref{eq:fcxx}}}
\newcommand{\fcs}{\ell_{\eqref{eq:fcs}}}
\newcommand{\Fcs}{L_{\eqref{eq:fcs}}}
\newcommand{\empFcs}{\empL_{\eqref{eq:fcs}}}

\newcommand{\epsemp}{\epsilon}

\newcommand{\Si}{S^{\setminus i}}
\newcommand{\rav}{\textrm{rav}}


\newcommand{\breg}[3]{\Delta_{#1}\left( #2\middle| #3 \right)}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\hL}{\hat{L}}
%\newcommand{\L}[1]{L\left(#1\right)}
\newcommand{\cL}{\mc{L}}
\newcommand{\hw}{\hat{\w}}
\newcommand{\eh}{\hat{h}}
%\newcommand{\hopt}{h^\star}
\newcommand{\Rad}{\mc{R}}
%\newcommand{\H}{\mc{H}}
\newcommand{\Z}{\mc{Z}}
\newcommand{\hRad}{\mc{R}}
\newcommand{\fat}{\mathrm{fat}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\herr}{\widehat{\mathrm{err}}}
%\newcommand{\F}{\mathcal{F}}
%\newcommand{\x}{\mbb{x}}
\newcommand{\Es}[2]{\mbb{E}_{#1}\left[ #2 \right]}
%\newcommand{\ip}[2]{{\left\langle{#1},{#2}\right\rangle}}
\newcommand{\B}{\mc{B}}
\newcommand{\Bd}{\mc{B}^{\star}}
\newcommand{\W}{\mc{W}}
\newcommand{\Wd}{\mc{W}^\star}
\renewcommand{\H}{\mc{H}}
\newcommand{\Hd}{\mc{H}^\star}
\renewcommand{\X}{\mc{X}}
\newcommand{\Val}{\mc{V}}
\newcommand{\Valstat}{\mc{V}^{\mrm{iid}}}
\newcommand{\Reg}{\mbf{Reg}}
\newcommand{\uVal}{\mc{V}^{\mathrm{unif}}}
\newcommand{\aVal}{\mc{V}^{\mathrm{avg}}}
\newcommand{\Xd}{\mc{X}^\star}
%\newcommand{\z}{\mbf{z}}
\newcommand{\En}{\mbb{E}}
\newcommand{\suptype}{p^\star}
%\newcommand{\L}{\mc{L}}
%\newcommand{\F}{\mc{F}}
\newcommand{\Algo}{\mc{A}}
\newcommand{\rAlgo}{\overline{\mc{A}}}
\newcommand{\uV}{V^{\mathrm{unif}}}
\newcommand{\V}{V}
\newcommand{\aV}{V^{\mathrm{avg}}}
\newcommand{\Algomd}{\mc{A}_{\mathrm{MD}}}
\newcommand{\Algosmd}{\overline{\mc{A}_{\mathrm{MD}}}}
\newcommand{\MD}{\mathrm{MD}}


\newcommand{\prightarrow}{\stackrel{\scriptscriptstyle P}{\rightarrow}}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\halgo}{\tilde{\h}} % h by algorithm
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\PD}{\mathcal P}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\QD}{\mathcal Q}
\newcommand{\balpha}{\mbf{\alpha}}
\newcommand{\phifunc}[1]{\phi\left(#1\right)}
\newcommand{\trm}[1]{\textrm{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\ip}[2]{\left<#1,#2\right>}

% General math
%\newcommand{\v}{\mbb{v}}
\newcommand{\sign}{\mrm{sign}}
\newcommand{\argmin}[1]{\underset{#1}{\mrm{argmin}} \ }
\newcommand{\argmax}[1]{\underset{#1}{\mrm{argmax}} \ }
\newcommand{\reals}{\mathbb{R}}
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]} % brackets
\newcommand{\Ebr}[1]{\mathbb{E}\left\{ #1 \right\}} % curly braces
%\newcommand{\En}{\mathbb{E}}  % no brackets or braces
%\newcommand{\Es}[2]{\mathbb{E}_{#1}\left[ #2 \right]} % subscript + brackets

\newcommand{\Ps}[2]{\mathbb{P}_{#1}\left[ #2 \right]}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\inner}[1]{\left\langle #1 \right\rangle}
\newcommand{\lv}{\left\|}
\newcommand{\rv}{\right\|}
\newcommand{\Phifunc}[1]{\Phi\left(#1\right)}
\newcommand{\ind}[1]{{\bf 1}_{\left\{#1\right\}}}
%\newcommand{\ind}[1]{\ 1\hspace{-2.3mm}{1}{\left\{#1\right\}}}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\newcommand{\eqdist}{\stackrel{\text{d}}{=}}
\newcommand{\alphT}{\widehat{\alpha}(T)}
\newcommand{\PF}{\mathcal P}
\newcommand{\QY}{\mathcal Q}
\newcommand{\jp}{\ensuremath{\mathbf{p}}}

% Bold symbols
\newcommand\s{\mathbf{s}}
%\newcommand\w{\mathbf{w}}
%\newcommand\x{\mathbf{x}}
%\newcommand\y{\mathbf{y}}
%\newcommand\z{\mathbf{z}}


\renewcommand\v{\mathbf{v}}

% Calligraphic symbols
\newcommand\cD{\mathcal{D}}
%\newcommand\X{\mathcal{X}}
%\newcommand\Y{\mathcal{Y}}
\renewcommand\Z{\mathcal{Z}}
\renewcommand\F{\mathcal{F}}
\newcommand\cH{\mathcal{H}}
\newcommand\bcH{\bar{\mathcal{H}}}
\newcommand\N{\mathcal{N}}
\newcommand\M{\mathcal{M}}
%\newcommand\W{\mathcal{W}}
\newcommand\Nhat{\mathcal{\widehat{N}}}

% Notations
\newcommand\ldim{\mathrm{Ldim}}
%\newcommand\fat{\mathrm{fat}}
\newcommand\Img{\mbox{Img}}
\newcommand\sparam{\sigma} % Strong convexity constant
\newcommand\Psimax{\ensuremath{\Psi_{\mathrm{max}}}}

% Calligraphic notations
%\newcommand\Rad{\mathfrak{R}}
%\newcommand\Val{\mathcal{V}}
\newcommand\Valdet{\mathcal{V}^{\mathrm{det}}}
\newcommand\Dudley{\mathfrak{D}}
%\newcommand\Reg{\mrm{Reg}}
\newcommand\D{\mc{D}}
\renewcommand\P{\mbf{P}}
\newcommand{\Prob}[1]{\mathbb{P}\left[ #1 \right]}


% For the examples section
\newcommand\Xcvx{\X_\mathrm{cvx}}
\newcommand\Xlin{\X_\mathrm{lin}}
%\newcommand{\loss}{\ell}
\newcommand{\Nature}{\emph{Nature}}
\newcommand{\Adversary}{\emph{Adversary}}
\newcommand{\Learner}{\emph{Learner} }
\renewcommand{\L}{L}
%\newcommand{\h}{h}
\renewcommand{\hL}{\widehat{L}}
\newcommand{\bnsp}{\mc{B}}
\renewcommand{\Algo}{\mbf{A}}
\newcommand{\Algostat}{\mbf{A}_{\mrm{stat}}}
\newcommand{\Algoonline}{\mbf{A}_{\mrm{online}}}
\newcommand{\OptAlgo}{\mrm{Alg}}
\newcommand\Ans{\mrm{I}}
\renewcommand\Lip{C}
\newcommand\Info{\mc{I}}
\newcommand\Oracle{\mc{O}}
\newcommand\epserm{\epsilon_{\mrm{erm}}}

\newcommand{\fatstat}{\fat^{\mrm{iid}}}
\newcommand{\faton}{\mathfrak{fat}^{\mrm{seq}}}
\newcommand{\Radstat}{\Rad^{\mrm{iid}}}
%\newcommand{\Radon}{\Rad^{\mrm{mart}}}
\newcommand{\Radon}{\mathfrak{R}^{\mrm{seq}}}
\newcommand{\Nstat}{\mathcal{N}^{\mrm{iid}}}
\newcommand{\Nonl}{\mathfrak{N}^{\mrm{seq}}}
\newcommand\Dudleystat{\mathfrak{D}^{\mrm{iid}}}
\newcommand\Dudleyon{\mathfrak{D}^{\mrm{seq}}}
%\newcommand\epsstable{\epsilon_{\mrm{stab}}}
%\newcommand\epscon{\epsilon_{\mrm{learn}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
